RT-HDIST: Ray-Tracing Core-based Hausdorff Distance Computation

The Hausdorff distance is a fundamental metric with widespread applications across various fields. However, its computation remains computationally expensive, especially for large-scale datasets. In this work, we present RT-HDIST, the first Hausdorff distance algorithm accelerated by ray-tracing cores (RT-cores). By reformulating the Hausdorff distance problem as a series of nearest-neighbor searches and introducing a novel quantized index space, RT-HDIST achieves significant reductions in computational overhead while maintaining exact results. Extensive benchmarks demonstrate up to a two-order-of-magnitude speedup over prior state-of-the-art methods, underscoring RT-HDIST's potential for real-time and large-scale applications.

==> 00_methods.tex <==

\Skip{
\section{RT-based Hausdorff Distance} \label{sec:method}

Previous works have used distance queries between primitives to compute the Hausdorff distance. However, implementing distance queries within ray tracing is not convenient and often requires complex methods. In this work, we compute the Hausdorff distance using nearest-neighbor approaches instead of the usual distance queries (Sec.~\ref{sec:method_sub_nn}). We also propose methods to accelerate the nearest-neighbor search and the computation of the Hausdorff distance by removing unnecessary operations.


\subsection{Overview}

Fig.~\ref{fig:Overview} presents an overview of our ray-tracing-based Hausdorff distance computation algorithms. The process is implemented based on RTNN with two proposed strategies. We firstly defined three primary problems to solve issues of RTNN works (Sec.~\ref{sec:problem_definition}), and then proposed the strategies focus on that.

Our process's first step is voxelization. In these steps, we divide the target points into uniform grids and cluster the points inside of same voxels. And then, we project the voxels to index space. These projected points will be representative points of the cluster. We build the Geometry Acceleration Structure (GAS) that is known as Bottom-Level Acceleration Structure (BLAS) in OptiX about the AABBs which has arbitrary box size and is centered on representative points (Sec.~\ref{sec:method_voxel_cluster}).

Next, we query the points and search for the nearest neighbor voxel of queries on the index space. The query points are also quantized by target voxel. To search for the nearest target, we adapt the elimination process of unnecessary points called "Filtering" and gradually expand the process of the search area called "Optimization" (Sec.~\ref{sec:method_filtering_optimization}). Finally, we compute the physical distance between query points and inner points of the nearest voxels.

Through this process, we get the Hausdorff distance $h(A,B)$.
}



\subsection{Problem definition} \label{sec:problem_definition}

The primary problems of nearest-neighbor based on ray tracing are:

\paragraph{AABB size} The accuracy and performance of the methods are influenced by the size of the AABB. If the AABB is selected too small, we will fail to find the correct nearest pair. On the other way, if the AABB is selected too big, the ray takes too much time to traverse the scene. However, these selection of the size of the AABB is difficult because suitable size is ambiguous for data type or relations of point-query sets.

\paragraph{Distance of two compare set} If the two point set is close enough, then the distance-based nearest neighbor is well-worked.  But on the contrary, if the two sets are far, then the size of the AABB needs to be a bigger size. In this case, the ray reports the intersection for almost all target points. This problem causes serious performance leaks.

\paragraph{Density of the point set} In this case, the target points are concentrated in too small a space. Even if we choose a small enough size of the AABB, the ray can be intersected for all of the AABBs. It may be more desirable to calculate the distance honestly.

We propose two strategies that focus on these primary problems.

\subsection{Quantized voxel cluster} \label{sec:method_voxel_cluster}

In the nearest neighbor search, too many points and queries often cause performance to decline. To minimize the number of computations, we clustered the points into representative points or voxels.

Our approach is to generate the AABBs above the representative points not all source points. These representative points are a "Cluster", that contains the original source points that construct the representative. During the traverse, the ray reports the intersection of AABB and includes information about representative points. These methods give two benefits. Which one is relieving the traverse time of acceleration structure about dense points by computing the distance to brute force per inner points of cluster. The other one is building explicit hierarchies for customizing. Currently, the ray tracing platform supports the implicit acceleration structure for ray tracing, therefore we can`t access the intermediate nodes of BVH. However, these approaches enable control on the intermediate node by forcing insertion of the node "Cluster".

To create a cluster, we first compute AABB for target points and then we divide the AABB uniformly with a suitable voxel count (In our implementations, we choose 6$\sim$8 bit count for each axis). The points try to contain the uniform grids, and those points are encoded to Morton codes. In the next step, we sort the points by Morton codes and remove the empty voxels. As a result, the voxels be "Cluster", which includes the information of pointers for start points with the same Morton codes.

Choosing the representative points for the cluster is difficult. Generally, we can choose the voxel center or centroid of inner points. But, in our implementations, our representative points are the voxel index. This voxel index can be replaced by the integer coordinates in uniform grid space that is constructed for each cell size has (1,1,1) cube. Therefore, each point going to become distant as much as at least 1. These results allow you to configure voxel sizes (1,1,1) of the same specification for any data type.

{\bf Error bound}: Even if we compute the neighbor cluster in voxel-index-space, the actual distance is calculated as the space of the original points.
Regarding the relationship between the nearest point and the nearest cluster, for a query point $q$, the nearest cluster $\square N$, and the nearest point $n$, we can establish the following inequality:
\begin{equation} \label{eq:error_bound_of_voxel}
    \min d(q, \square N) \leq d(q, n) \leq \max d(q, \square N)
\end{equation}
This inequality indicates that the distance from $q$ to the nearest point $n$ lies between the minimum and maximum distances from $q$ to all points in the cluster $\square N$. Thus, the nearest point $n$ exists within the voxel diagonal distance of the nearest cluster $\square N$. That is why we must investigate the neighbor voxel of $\square N$ to cover error bounds not only  $\square N$. These results can be computed by choosing AABB size to $a \sqrt{3}$, where $a$ is a hyperparameter that is the expected closest distance as $\min d(q, \square N)$.

\subsection{Filtering and Optimization} \label{sec:method_filtering_optimization}

Although our implementation employs a nearest neighbor search approach to compute the Hausdorff distance, computing the nearest neighbor for every point is not strictly necessary. In fact, attempting to do so imposes a significant computational overhead. To alleviate this issue, we introduce a “filtering” mechanism to eliminate superfluous candidates and an “optimization” technique that identifies Hausdorff candidates through a gradual filtering process.

The "filtering" strategy is similar to the Filter-Refine framework which is a general framework for search problem~\cite{mandarapu2024arkade}. The most basic strategy is inferring the candidates set from the data and then computing the distance between the query and the subset of them. In contrast to Mandarapu's methods~\cite{mandarapu2024arkade}, our filtering strategy only checks whether the query did intersected with the AABB or not. Because our objective is computing the Hausdorff distance, therefore we can cull the unnecessary points by setting the lower bound $\underline{h}(A,B)$ to filtering box size (See also Fig.~\ref{fig:comparison_of_filtering}). Finally, we compute the distance between non-eliminated query points and target points. In this step also adapted the Filter-Refine approaches, we set the upper bound filtering box that has $\overline{h}(A,B)$ and then compute the distance when intersect is called (Fig.~\ref{fig:ours_filter_optimiziation}).

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Image/filtering_nn.pdf}
        \caption{Nearest neighbor filtering}
        \label{fig:arkade_filter_refine}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Image/filtering_hd.pdf}
        \caption{Ours}\label{fig:ours_filter_optimiziation}
    \end{subfigure}
    \hfill
    \caption{Comparison of filtering methods. The blue points mean target points and the orange points mean query points. The dotted box means a filtering box. The red line is computing candidates for the final results. The prior RTNN approach (a) checks the inside of the filter box and computes the distance of inside points. Our approach (b) eliminates the points when the intersected point first hits, and then launches the RTNN after increasing the box.
    }
    \label{fig:comparison_of_filtering}
\end{figure}

The biggest challenge of ray-tracing-based nearest neighbor search such as RTNN and Arkade~\cite{zhu2022rtnn,mandarapu2024arkade} is choosing the radius of the search area. They use the size of complicatedly-calculated megacell~\cite{zhu2022rtnn} or pre-calculated or arbitrarily defined initial box sizes~\cite{nagarajan2023trueknn, mandarapu2024arkade}. To be free from the limitation of choosing the search radius $\epsilon$, we propose the optimization process that progressively eliminates the candidates by increasing the initial box size.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Image/boundary condition.pdf}
    \caption{Optimization process and boundary condition. The red dotted box means $i^{th}$ and the yellow dotted box means $i+1^{th}$ iteration box. The query point that is inside of $i^{th}$ one is removed during the process, therefore the next intersected points are only the boundary points of $i+1^{th}$ box (In other words, that points exist between $i^{th}$ and $i+1^{th}$ boxes).
    }
    \label{fig:boundary_condition}
\end{figure}

In our implementation, the initial box size is $\sqrt{3}$ because our filtering process is worked on the voxel index space (as mentioned in Sec.~\ref{sec:method_voxel_cluster}). In fact, the query point is quantized by the target's voxelized condition, and then the physical distance on the Integer space is always determined to be less than $a\sqrt{3}$. That reason why, we grow the box per iteration as much as $\sqrt{3}$, and filter the hit query points until there are no remaining non-hit query points. As shown in Fig.~\ref{fig:boundary_condition}, the intersected query point of each iteration always exists in the boundary of $i^{th}$ boxes. So the number of intersections for query points is increased to a minimum at each iteration. To enhance the performance, we uses the reduction operation~\cite{roger2007efficient} on the GPU to eliminate the intersected queries.
Finally, when no more queries are left, we traverse once again for the remaining queries in the previous iteration and calculate the Hausdorff distance between them and the target.

\input{Context/Algorithm/Filtering-Optimization process}

The overall process of proposed Filtering-Optimization can be seen in Algorithm~\ref{algo:filtering-optimization process}.

\paragraph{Error bound momentum:} The error bound is $\sqrt{3}$ in the index space because the nearest point exists on the neighbor of the nearest voxel as defined in the equation~\ref{eq:error_bound_of_voxel}. Therefore, we increase the box size once again for only the computing phase, by doing this, most errors are resolved.

\paragraph{Observation:} We build AS for the inner point cloud of the cluster and test it. However, the building overhead of AS per cluster takes time too much than when computing naive distance in a shader program. Therefore we present this issue for hierarchical processing in future work.

==> Context/Algorithm/Filtering-Optimization_process.tex <==
\begin{algorithm}
    \caption{Filtering-Optimization process} \label{algo:filtering-optimization process}

    \begin{algorithmic}[1]

    \State \textbf{Input:} Target set $P$ and Query set $Q$
    \State \textbf{Output:} One-way Hausdorff distance $h(P,Q)$

    \medskip

    \State queries $\leftarrow Q$
    \State remain $\leftarrow Q.\text{size}$
    \State representative $\leftarrow$ buildCluster($P$)
    \State eps $\leftarrow \sqrt{3}$
    \State GAS $\leftarrow$ build(representative, eps)

\While{remain $>$ 0}
    \State GAS $\leftarrow$ refit(representative, eps)
    \State isHit $\leftarrow$ traverse(queries, GAS, state $=$ Filtering)
    \State eps $\leftarrow$ eps + $\sqrt{3}$
    \State reduced $\leftarrow$ reduce(queries, isHit)

    \If{reduced.\text{size} $=$ 0}
        \State GAS $\leftarrow$ refit(representative, eps)
        \State distance $\leftarrow$ traverse(queries, GAS, state $=$ Computing)
        \State $h(P,Q)$ $\leftarrow$ max(distance)
    \Else
        \State queries $\leftarrow$ reduced
        \State remain $\leftarrow$ reduced.\text{size}
    \EndIf
\EndWhile

\State \Return $h(P,Q)$
\end{algorithmic}
\end{algorithm}


==> Context/Figure/RTNN.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Image/rtnn_process.pdf}
        \caption{}
        \label{fig:rtnn_process}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Image/macrocell-partioning-based-e.pdf}
        \caption{}\label{fig:macro-cell-based-multi-as}
    \end{subfigure}
    \hfill
    \caption{RTNN process. (a) To compute $\epsilon$-neighbor search, firstly the AABB that has the size of $\epsilon$ builds per each target point. Next, the compute intersection of the query and AABB, if they hit, then check within distance $\epsilon$. If queries are within, that query is a neighbor. (b) Multi-acceleration structure system using macro cell grid partitioning. The first step is the insertion of the target point into the macro cell grid. If the number of inner points of the cell, then the cell box extends until the number of inner points reaches $k$. Each color means the same box sizes and the acceleration hierarchy was built as much as the number of colors (For this example, there is a total of three AS for each $\epsilon$ is 3,5,7).
    }
    \label{fig:rtnn}
\end{figure}

==> Context/Table/error_comparison.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\caption{Result comparison with previous works. The values in parentheses indicate error rates. *Note that this result was obtained regardless of k and GPU device.}
\centering
\label{tb:distane_comparison_with_previous}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
                           & Overlap & Translated & Zheng~\cite{zheng2022economic}                                                     & Sacht~\cite{sacht2024cascading}                                                     & Ours                                                           &                            & Overlap & Translated & Zheng~\cite{zheng2022economic}                                                     & Sacht~\cite{sacht2024cascading}                                                     & Ours                                                           \\ \hline \hline
    \multirow{5}{*}[-5.5ex]{Bunny} & 0.1     & 8.76       & \begin{tabular}[c]{@{}c@{}}8.76\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}8.76\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}8.76\\(0.01\%)\end{tabular}   & \multirow{5}{*}[-5.5ex]{David}     & 0.1     & 16.56      & \begin{tabular}[c]{@{}c@{}}16.56\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}16.56\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}16.56\\(0.00\%)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                           & 0.3     & 4.66       & \begin{tabular}[c]{@{}c@{}}4.66\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4.66\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4.66\\(0.01\%)\end{tabular}   &                            & 0.3     & 7.50       & \begin{tabular}[c]{@{}c@{}}7.50\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}7.50\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}7.50\\(0.00\%)\end{tabular}   \\ \cline{2-6} \cline{8-12} 
                           & 0.5     & 2.48       & \begin{tabular}[c]{@{}c@{}}2.48\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.48\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}2.48\\(0.03\%)\end{tabular}   &                            & 0.5     & 3.56       & \begin{tabular}[c]{@{}c@{}}3.56\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.56\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3.56\\(0.00\%)\end{tabular}   \\ \cline{2-6} \cline{8-12} 
                           & 0.7     & 1.18       & \begin{tabular}[c]{@{}c@{}}1.18\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.18\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.18\\(0.09\%)\end{tabular}   &                            & 0.7     & 1.75       & \begin{tabular}[c]{@{}c@{}}1.75\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.75\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1.75\\(0.00\%)\end{tabular}   \\ \cline{2-6} \cline{8-12} 
                           & 0.9     & 0.33       & \begin{tabular}[c]{@{}c@{}}0.33\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.33\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.34\\(0.77\%)\end{tabular}   &                            & 0.9     & 0.50       & \begin{tabular}[c]{@{}c@{}}0.50\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.50\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0.50\\(0.00\%)\end{tabular}   \\ \hline \hline
    \multirow{5}{*}[-5.5ex]{Lucy}  & 0.1     & 214.86     & \begin{tabular}[c]{@{}c@{}}214.86\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}214.86\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}214.86\\(0.00\%)\end{tabular} & \multirow{5}{*}[-5.5ex]{Stmatthew} & 0.1     & 643.06     & \begin{tabular}[c]{@{}c@{}}643.06\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}643.06\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}643.06\\(0.00\%)\end{tabular} \\ \cline{2-6} \cline{8-12} 
                           & 0.3     & 116.21     & \begin{tabular}[c]{@{}c@{}}116.21\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}116.21\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}116.21\\(0.00\%)\end{tabular} &                            & 0.3     & 385.17     & \begin{tabular}[c]{@{}c@{}}385.17\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}385.17\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}385.17\\(0.00\%)\end{tabular} \\ \cline{2-6} \cline{8-12} 
                           & 0.5     & 57.48      & \begin{tabular}[c]{@{}c@{}}57.48\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}57.48\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}57.48\\(0.00\%)\end{tabular}  &                            & 0.5     & 225.27     & \begin{tabular}[c]{@{}c@{}}225.27\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}225.27\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}225.27\\(0.00\%)\end{tabular} \\ \cline{2-6} \cline{8-12} 
                           & 0.7     & 25.93      & \begin{tabular}[c]{@{}c@{}}25.93\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}25.93\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}25.93\\(0.00\%)\end{tabular}  &                            & 0.7     & 111.57     & \begin{tabular}[c]{@{}c@{}}111.57\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}111.57\\(0.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}111.57\\(0.00\%)\end{tabular} \\ \cline{2-6} \cline{8-12} 
                           & 0.9     & 7.17       & \begin{tabular}[c]{@{}c@{}}7.17\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}7.17\\(0.00\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}7.17\\(0.00\%)\end{tabular}   &                            & 0.9     & 31.45      & \begin{tabular}[c]{@{}c@{}}31.45\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}31.45\\(0.00\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}31.45\\(0.00\%)\end{tabular}  \\ \hline \hline
    \end{tabular}%
    }
    \end{table*}


==> Context/Table/old_tables.tex <==
\Skip{
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\caption{Benchmarks.}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|c}
\hline
Dataset          & Armadillo   & Happy Buddha   & Dragon  \\ \hline \hline
Number of vertex & 172,974 & 543,652 & 437,645 \\ \hline
Number of triangles &  345,944     &   1,087,716     &   871,414 \\ \hline
      Image            
& \raisebox{-.5\height}{\includegraphics[width=0.3\textwidth]{Image/Dataset/crop_armadilo.png}}
& \raisebox{-.5\height}{\includegraphics[width=0.3\textwidth]{Image/Dataset/crop_budda.png}}   
&  \raisebox{-.5\height}{\includegraphics[width=0.3\textwidth]{Image/Dataset/crop_dragon.png}}
\\ \hline
Dataset          &  Lucy & Thai Statue & Asian Dragon  \\ \hline \hline
Number of vertex  & 14,027,872 & 4,999,996 & 3,609,600 \\ \hline
Number of triangles &   28,055,742     & 10,000,000 &  7,219,045 \\ \hline
      Image     
&  \raisebox{-.5\height}{\includegraphics[width=0.3\textwidth]{Image/Dataset/crop_lucy.png}}     
&  \raisebox{-.5\height}{\includegraphics[width=0.3\textwidth]{Image/Dataset/crop_tistattuew.png}}          
&  \raisebox{-.5\height}{\includegraphics[width=0.3\textwidth]{Image/Dataset/crop_xyzdragon.png}}     
\\ \hline
\end{tabular}%
}
\label{tb:dataset}
\end{table*}
}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[hbt!]
\small
\caption{Decimates}
\centering
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{Data} & \multicolumn{2}{c|}{Original}   & \multicolumn{2}{c|}{Decimates}  \\ \cline{2-5} 
                      & \multicolumn{1}{c|}{Vert} & Tri & \multicolumn{1}{c|}{Vert} & Tri \\ \hline
Happy Buddha          & \multicolumn{1}{c|}{543,652}     & 1,087,716    & \multicolumn{1}{c|}{26,986}     & 54,384    \\ \hline
Dragon                & \multicolumn{1}{c|}{437,645}     & 871,414    & \multicolumn{1}{c|}{22,632}     & 43,570    \\ \hline
Thai Statue           & \multicolumn{1}{c|}{4,999,996}     & 10,000,000    & \multicolumn{1}{c|}{9,996}     & 20,000   \\ \hline
Asian Dragon          & \multicolumn{1}{c|}{3,609,600}     & 7,219,045    & \multicolumn{1}{c|}{10,830}     & 21,656    \\ \hline
\end{tabular}%
\label{tb:decimates_info}
\end{table}

\begin{table}[hbt!]
\small
\caption{Decimates performance(s). (Buddha, Dragon, Statue k=8, Asian Dragon K=7)}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Data                  & Zheng & Pompeiu & Ours \\ \hline
Happy Buddha          & 9.67      &  3.69       & 0.04 \\ \hline
Dragon                & 8.92      &  3.47       & 0.04 \\ \hline
Thai Statue           & 27.46      & 16.01        & 0.08 \\ \hline
Asian Dragon          & 21.08      & 8.90        & 0.10 \\ \hline
\end{tabular}%
\label{tb:decimates_time}
\end{table}

==> Context/Table/performance_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\caption{Performance comparison with previous works. The performance is in seconds. The values in parentheses indicate the amount of speed-up than Zheng~\cite{zheng2022economic}. *Note that our performance is the result obtained using best k for each scenario in RTX 4080 (Happy buddha k = 7, Dragon, Thai Statue, Asian Dragon k=8).}
\centering
\label{tb:performance_comparison_with_previous}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
                           & Translated ratio & Translated & Zheng~\shortcite{zheng2022economic}          & Sacht~\shortcite{sacht2024cascading}         & Ours                                                           &                            & Translated ratio & Translated & Zheng~\shortcite{zheng2022economic}          & Sacht~\shortcite{sacht2024cascading}         & Ours                                                          \\ \hline \hline
      \multirow{5}{*}[-5.5ex]{Dragon}                                                & 0.1              & 0.020489   & \begin{tabular}[c]{@{}c@{}}3.90\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.39\\(x1.63)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.09\\(x42.17)\end{tabular} & \multirow{5}{*}[-5.5ex]{\begin{tabular}[c]{@{}c@{}}Happy\\ Buddha\end{tabular}} & 0.1     & 0.008132   & \begin{tabular}[c]{@{}c@{}}5.67\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.67\\(x2.13)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.34\\(x16.75)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.3              & 0.061467   & \begin{tabular}[c]{@{}c@{}}3.71\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.31\\(x1.61)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.13\\(x28.63)\end{tabular} &                                                                         & 0.3     & 0.024397   & \begin{tabular}[c]{@{}c@{}}4.62\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.87\\(x1.61)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.15\\(x30.95)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.5              & 0.102445   & \begin{tabular}[c]{@{}c@{}}3.72\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.42\\(x1.54)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.20\\(x18.84)\end{tabular} &                                                                         & 0.5     & 0.040661   & \begin{tabular}[c]{@{}c@{}}4.53\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.88\\(x1.57)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.13\\(x35.44)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.7              & 0.143423   & \begin{tabular}[c]{@{}c@{}}3.69\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.27\\(x1.63)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.26\\(x14.18)\end{tabular} &                                                                         & 0.7     & 0.056925   & \begin{tabular}[c]{@{}c@{}}4.61\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.87\\(x1.60)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.16\\(x29.55)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.9              & 0.184401   & \begin{tabular}[c]{@{}c@{}}3.75\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.15\\(x1.75)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.25\\(x15.15)\end{tabular} &                                                                         & 00.9    & 0.07319    & \begin{tabular}[c]{@{}c@{}}4.56\\(x1.00)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.88\\(x1.58)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.19\\(x23.63)\end{tabular}  \\ \hline
\multirow{5}{*}[-5.5ex]{\begin{tabular}[c]{@{}c@{}}Thai\\ Statue\end{tabular}} & 0.1              & 23.5224    & \begin{tabular}[c]{@{}c@{}}50.87\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.40\\(x1.52)\end{tabular} & \begin{tabular}[c]{@{}c@{}}10.45\\(x4.87)\end{tabular} & \multirow{5}{*}[-5.5ex]{\begin{tabular}[c]{@{}c@{}}Asian\\ Dragon\end{tabular}} & 0.1     & 20.1744    & \begin{tabular}[c]{@{}c@{}}33.53\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.97\\(x1.40)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.30\\(x111.40)\end{tabular} \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.3              & 70.5672    & \begin{tabular}[c]{@{}c@{}}50.28\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}41.32\\(x1.22)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.77\\(x65.23)\end{tabular} &                                                                         & 0.3     & 60.5231    & \begin{tabular}[c]{@{}c@{}}33.41\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}25.33\\(x1.32)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.54\\(x61.73)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.5              & 117.612    & \begin{tabular}[c]{@{}c@{}}50.13\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}43.18\\(x1.16)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.00\\(x50.01)\end{tabular} &                                                                         & 0.5     & 100.872    & \begin{tabular}[c]{@{}c@{}}33.36\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}25.10\\(x1.33)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.41\\(x82.09)\end{tabular}  \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.7              & 164.657    & \begin{tabular}[c]{@{}c@{}}50.37\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}43.56\\(x1.16)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.77\\(x28.43)\end{tabular} &                                                                         & 0.7     & 141.22     & \begin{tabular}[c]{@{}c@{}}33.38\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.09\\(x1.39)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.25\\(x135.80)\end{tabular} \\ \cline{2-6} \cline{8-12} 
                                                                       & 0.9              & 211.702    & \begin{tabular}[c]{@{}c@{}}50.46\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}44.36\\(x1.14)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.74\\(x18.43)\end{tabular} &                                                                         & 0.9     & 181.569    & \begin{tabular}[c]{@{}c@{}}33.42\\(x1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.19\\(x1.44)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.21\\(x157.86)\end{tabular} \\ 
                                                                       \hline
     \hline
\end{tabular}%
}
\end{table*}
